FL-NAS: Towards Fairness of NAS for Resource Constrained Devices via Large Language Models

Neural Architecture Search (NAS) has become the de fecto tools in the industry in automating the design of deep neural networks for various applications, especially those driven by mobile and edge devices with limited computing resources. The emerging large language models (LLMs), due to their prowess, have also been incorporated into NAS recently and show some promising results. This paper conducts further exploration in this direction by considering three important design metrics simultaneously, i.e., model accuracy, fairness, and hardware deployment efficiency. We propose a novel LLM-based NAS framework, FL-NAS, in this paper, and show experimentally that FL-NAS can indeed find high-performing DNNs, beating state-of-the-art DNN models by orders-of-magnitude across almost all design considerations.

==> 1_Intro.tex <==
\section{Introduction}

% =====version 1
% In the rapidly evolving landscape of deep learning, Neural Architecture Search (NAS) \cite{elsken2019neural} has emerged as a cornerstone, offering the promise of automating the design of neural network architectures. \textcolor{blue}{yuting: Neural Architecture Search (NAS) \cite{elsken2019neural} has arisen as a pivotal innovation, holding the potential to revolutionize the automated design of neural network architectures.} Its potential to consistently deliver high-performing models across diverse tasks is undeniable. However, NAS comes with its own set of challenges. The cost of performing a task-specific neural network search is becoming overwhelming high to prevent its further development. \textcolor{blue}{yuting: The exorbitant computing cost of performing a task-specific neural network search impedes its further advancement.} Various works have been conducted to accelerate NAS. \textcolor{blue}{yuting: Numerous research efforts have been undertaken to expedite NAS process. For example, in \cite{pham2018efficient}, the authors proposed to share trained model parameters in the same model components to reduce searching expense. On the other hand, to better evaluate the searched models, this paper \cite{liu2018darts} shows the effectiveness of using differentiable model architectures. Moreover, devising a fast searching algorithm \cite{li2020random}  is also a valuable direction to accelerate NAS. } For example, the model trained parameters \cite{pham2018efficient} can be shared for same model components to accelerate the model searching, the architecture can also be designed to be differentiable \cite{liu2018darts} for better searched model evaluation, and design the better search algorithm \cite{li2020random} is also a way to accelerate NAS. However, for these works regarding accelerate the speed of searching the optimal neural network, overwhelm computational resources and time are need to perform. This is because the classical NAS replies on recurrent neural network (RNN) controller \cite{zoph2016neural} to search for the new model component and update the searched model. This RNN structure is actually a fancy for-loop. \textcolor{blue}{yuting: However, the classical NAS \cite{zoph2016neural} method applies RNN controller to update the architecture hyperparameter searching space, which is a highly time-consuming process due to its inside for-loop manner. In addition to the consideration of network search speed, it is paramount to acknowledge the significance of computational resources limitations at the hardware infrastructure level.}

% ======version2
% In the rapidly evolving landscape of deep learning, Neural Architecture Search (NAS) \cite{elsken2019neural} has emerged as a cornerstone, offering the promise of automating the design of neural network architectures. Its potential to consistently deliver high-performing models across diverse tasks is undeniable. However, NAS comes with its own set of challenges. The cost of performing a task-specific neural network search is becoming overwhelming high to prevent its further development. Numerous research efforts have been undertaken to expedite NAS process. For example, in \cite{pham2018efficient}, the authors proposed to share trained model parameters in the same model components to reduce searching expense. On the other hand, to better evaluate the searched models, this paper \cite{liu2018darts} shows the effectiveness of using differentiable model architectures. Moreover, devising a fast searching algorithm \cite{li2020random} is also a valuable direction to accelerate NAS. However, the classical NAS \cite{zoph2016neural} method applies RNN controller to update the architecture hyperparameter searching space, which is a highly time-consuming process due to its inside for-loop manner. In addition to the consideration of network search speed, it is paramount to acknowledge the significance of computational resources limitations at the hardware infrastructure level.

As the rapid development of deep neural network (DNN), Neural Architecture Search (NAS) has emerged as a pivotal innovation, holding the potential to revolutionize the automated design of DNN architectures. Its ability to consistently produce high-performing DNN across diverse tasks is undeniable. However, the computational cost associated with NAS, especially when tailored for specific tasks, is becoming prohibitively high, hindering its further development.

% Several strategies have been proposed to expedite the NAS process. For instance, \cite{pham2018efficient} suggests sharing trained model parameters for identical components to accelerate the search. Making architectures differentiable can enhance the evaluation of searched models, as demonstrated by \cite{liu2018darts}. Additionally, \cite{li2020random} highlights the importance of devising faster search algorithms as a means to hasten NAS. However, these methods, despite their merits, still demand substantial computational resources and time. This is largely because classical NAS relies on a Recurrent Neural Network (RNN) controller~\cite{zoph2016neural} to search for new model components and update the searched model. This RNN structure essentially operates as a sophisticated for-loop.

% ====== version 1
% At the same time, as the development of AI democratization, we are seeing the increasing demand of deploying machine learning models which are backed by neural network into user-end device such as medical diagnostics system \cite{kaissis2020secure}, healthcare device \cite{jia2023importance}, and biosignal-monitor device \cite{jia2023addressing}. Unlike cloud and computing cluster based machine learning platform, which can access large-scale computational resources and train the machine learning model with huge volume of user data, the machine learning models on user-end device, while provides higher data privacy, can be short in limited computational resources and model unfairness issues. The existing works address these issues with model compression, model quantization, and hardware/software co-design \cite{han2015deep, yan2022reliability, yan2022swim, nagel2021white}. Unfortunately, these existing works purse the overall accuracy performance and ignore person-level accuracy across all diverse groups, where the person-level performance can be measured by fairness score. For example, in examining the skin cancer in ISIC \cite{gutman2016skin} dataset, a model embedded into a user-end device can have 44\% accuracy for young people, 73\% for adult, 65\% for male, and 58\% for female, even if this model can have 70\% overall accuracy.
Simultaneously, with the rise of AI democratization, there's an escalating demand to deploy machine learning models, underpinned by DNN, onto user-end devices. 
These devices can encompass medical diagnostic systems \cite{kaissis2020secure} and healthcare devices \cite{jia2023importance}.
In contrast to cloud and computing cluster-based platforms, which harness vast computational resources and train DNN on extensive user data, DNN on user-end devices, though offering enhanced data privacy, often grapple with constrained computational resources and fairness issues. Current research addresses these challenges through DNN compression, DNN quantization, and hardware/software co-design \cite{yan2022reliability, yan2022swim}. 
% \st{Regrettably, many of these solutions prioritize overall accuracy, sidelining person-level accuracy across diverse groups—a metric that can be gauged using fairness scores. For instance, when analyzing skin cancer using the ISIC dataset \cite{isic2019}, a DNN on a user-end device might achieve accuracies of 44\% for the young, 73\% for adults, 65\% for males, and 58\% for females, even if its overall accuracy stands at 70\%.}

Regrettably, many of these solutions prioritize overall accuracy while simultaneously neglecting to ensure an equitable distribution of results among various groups or individuals, a performance metric commonly known as the fairness score. In spite of the requirements for the NAS approach on performance adherence, various end-user devices post challenges on the viability of searched architectures.

% ====== version 1
% Other than optimizing the task-specific machine learning system which requires sophisticated design and operation as we mentioned above, directly searching the appropriate model considering the task-specific constraints can be a more viable approach. While the idea of NAS can perfectly fit this task, the difficulties remain in encoding the task-specific constraints into the RNN controller. First, the differences among different user-end devices can be huge. It's hard to design a unified standard to cover all the special properties of each device and convert these properties into search constraints. For example, wearing device can be memory limited \cite{ajani2021overview} and cannot load large-scale model. Furthermore, the device-specific task is more easily interpret into context-based search constraints, which cannot be encoded into the classical NAS RNN controller.
% \st{Rather than solely optimizing task-specific systems, a more promising approach might be to directly search for neural architecture that inherently consider task-specific constraints. While NAS aligns well with this idea, integrating these constraints into the RNN controller presents challenges. The heterogeneity of user-end devices complicates the creation of a universal standard that encapsulates the unique attributes of each device. For instance, wearables might be memory-constrained, making it challenging to accommodate large DNN. Moreover, device-specific tasks often translate into context-based constraints, which are not easily integrated into traditional NAS RNN controllers.}

% ====== version 1
% In response to these difficulties regarding search the appropriate model towards user-end device, we propose to employ Large Language Models (LLMs) to replace the RNN controller of classical NAS. LLMs, trained on extensive volume of human-generated text content, have a extraordinarily broad knowledge domain and language semantic understanding capabilities. Take these advantages, LLMs have already been used to design models and architectures \cite{yan2023viability} in computing search. As LLMs are interacted by prompts, the user-end information can be encoded into prompts which can be used to search the proper machine learning models to satisfy the user-specific requirements. In this case, LLMs act as the RNN controller to update the machine learning models. Better than RNN controller, LLMs can be better consider the machine learning models in a global perspective and have a wide domain knowledge. Furthermore, LLMs can understand high-level concept of fairness and consider it as constraint when design the model. Hence, LLMs perfectly fit to situation where the fairness is important due to user-level usage and the resource limitation, which means the user-specific situation can also be considered.
Rather than solely optimizing task-specific systems, a more promising approach might entail the direct exploration of neural architectures with inherent consideration of task-specific constraints. Diverse end-user devices complicate the establishment of a universal standard to accommodate various attributes of each device, which makes device-context constraints hard to assimilate into conventional NAS RNN controllers. Moreover, the search process of traditional NAS with a RNN controller to generate model hyperparameters can be computationally expensive, leading to substantial time and resource consumption. 

As powerful tools across diverse domains, LLMs have exhibited impressive capability in code generation, demonstrating their substantial promise in DNN and architecture design~\cite{yan2023viability}. Since designing architectures requires massive expert domain knowledge, LLMs expose their priorities with massive amounts of machine learning code they have been trained on. Interacting with LLMs through prompts allows for the encoding of user-end information such as the hardware resources and storage, facilitating the search for DNN that meet user-specific needs, which makes LLMs particularly suitable for task-specific systems with contains on fairness, resource limitations, etc.

% To address these challenges, we propose replacing the RNN controller in classical NAS with Large Language Models
% (LLMs). Trained on vast amounts of human-generated content, LLMs boast an expansive knowledge domain and exceptional
% language understanding. They have already demonstrated their prowess in DNN and architecture design [6]. Interacting with
% LLMs through prompts allows for the encoding of user-end information, facilitating the search for DNN that meet
% user-specific needs. LLMs, with their global perspective and extensive domain knowledge, can also comprehend the high-
% level concept of fairness, making them ideal for scenarios where fairness and resource limitations are paramount.

% % In this work, we introduce such a framework that have LLMs to take the place of RNN controller in classical NAS to enlighten an efficient way of implementing the idea of NAS and validate the framework capability of design neural architecture with hardware efficiency and high performance in accuracy and fairness. Our experimental results indicate substantial improvements: up to 18X reduction of parameter size, up to 4X reduction of inference latency, up to 55X reduction of memory space, up to 3.67\% improve of accuracy, and up to 18X reduction of unfairness score compared to the state-of-the-art (SOTA) FaHaNa \cite{sheng2022larger} under the same experimental settings.
% In this work, we introduce a framework that utilizes LLMs to replace the RNN controller traditionally used in classi-
% cal NAS, thereby illuminating a more efficient approach to implementing NAS concepts. This adjustment also aims to
% validate the framework’s ability to design DNN with enhanced hardware efficiency, accuracy, and fairness. Our experimental results demonstrate substantial improvements compared to the state-of-the-art (SOTA) works under identical experimental settings:
Aiming at fulfilling task-specific limitations in diverse end-user devices, this paper introduces a novel NAS approach, leveraging the LLMs' powerful potential. We empirically validate our approach's ability to design DNN with enhanced hardware efficiency, accuracy, and fairness. The experimental results demonstrate substantial improvements compared to the state-of-the-art (SOTA) works under identical experimental settings:
up to 18X reduction in parameter size, up to 4X reduction in inference latency, up to 55X reduction in memory space, up to 11.4\% improvement in accuracy, and up to 18X reduction in unfairness score.

% The rest of the paper structured as follows. Section 2 elaborates the background and explains our motivations. Section 3 demonstrates the details of this framework, its prompt template, and its search strategy. Section 4 illustrate the evaluation metrics used in the experiments and analysis of the experimental results. Section 5 provides the conclusion.
The remainder of the paper is structured as follows: Section 2 elaborates on the background and explains our motivations. Section 3 delineates the details of this framework, its prompt template, and its search strategy. Section 4 illustrates the evaluation metrics used in the experiments and provides an analysis of the experimental results. Section 5 presents the conclusion.


==> 2_Related.tex <==
\section{Related Works and Motivations}
\label{sec_background}

\subsection{Neural Architecture Search}

Early NAS research commonly employs evolutionary algorithms (EAs) and reinforcement learning (RL) to produce architectures. RL-based NAS methods utilize reinforcement learning algorithms like deep Q-learning and policy gradient methods, effectively guiding the search process towards optimal architectures, as evidenced by seminal works 
% \cite{zoph2016neural}, 
\cite{baker2017accelerating}. Conversely, EA-based NAS techniques \cite{liu2021survey} utilize principles from evolutionary computation, employing mutation, recombination, and selection to evolve neural architectures. These approaches demonstrate the ongoing pursuit within the NAS domain to balance effective exploration of intricate architecture spaces with computational efficiency. More recently, proxy-based NAS methods
% \cite{cai2018proxylessnas}, 
\cite{zhou2020econas} have gained attention for streamlining the architecture search process through surrogate models or performance predictors, aiming to expedite exploration by leveraging proxy metrics such as validation accuracy or computational cost.
% Several strategies have been proposed to expedite the NAS process. For instance, \cite{pham2018efficient} suggests sharing trained model parameters for identical components to accelerate the search. Making architectures differentiable can enhance the evaluation of searched models, as demonstrated by \cite{liu2018darts}. Additionally, \cite{li2020random} highlights the importance of devising faster search algorithms as a means to hasten NAS. However, these methods, despite their merits, still demand substantial computational resources and time. This is largely because classical NAS relies on a Recurrent Neural Network (RNN) controller~\cite{zoph2016neural} to search for new model components and update the searched model. This RNN structure essentially operates as a sophisticated for-loop.

% \st{Several strategies  have been proposed to expedite the NAS process. For instance, sharing trained DNN parameters for identical components to accelerate the search, making architectures differentiable can enhance the evaluation of searched neural architecture, and highlights the importance of devising faster search algorithms as a means to hasten NAS. However, these methods, despite their merits, still demand substantial computational resources and time. This is largely because classical NAS relies on a Recurrent Neural Network (RNN) controller to search for new DNN components and update the searched neural architectures. This RNN structure essentially operates as a sophisticated for-loop.}

\subsection{NAS via Large Language Models}

% With clear awareness of the lacks of conventional NAS, implementing the idea of NAS in different ways has been considered. As the rising of Large Language Models (LLMs), utilizing LLMs to accelerate the neural architecture searching speed and optimize the searching performance has been explored. The current most widely used advanced LLM is GPT-4 \cite{OpenAI2023GPT4TR}, whose logical inference capability on various professional \cite{bevilacqua2023automated} and academic benchmarks are superior than most existing language models such as Llama \cite{touvron2023llama}, Pythia \cite{biderman2023pythia}, and PaLM 2 \cite{anil2023palm}. Different from classical transformer-based models \cite{devlin2018bert, liu2019roberta, sanh2019distilbert}, and their related works \cite{qin2021ibert, luo2020open}, LLMs have expontially larger trainable parameters: Llama has 65B, GPT-3 has 175B, PaLM has 540B, and GPT-4 has 1.76T. With such a huge volume of trainable parameters, LLMs incorporate Mixture of Exports (MoEs) \cite{artetxe2021efficient} techniques and train on overwhelming large high quality datasets. For example, Llama is trained on the dataset consists of CCNet [67\%], C4 [15\%], GitHub [4.5\%], Wikipedia [4.5\%], Books [4.5\%], ArXiv [2.5\%], Stack Exchange[2\%] \cite{touvron2023llama}. All of these give LLMs capability of wide domain knowledge to design and optimize neural architecture to satisfy user-specific tasks.

% GENIUS \cite{zheng2023can} is the first work investigate the potential of utilizing GPT-4 to perform NAS. GENUIS uses GPT-4 as a "black box" with domain knowledge relevant to neural architecture design. This "black box" is drived by prompts, which only give GPT-4 a broad and vague scope of search and ask GPT-4 to consider the accuracy only. Furthremore, GPT4GNAS \cite{wang2023graph} also explore the potential of LLMs in Graph Neural Architecture Search (GNAS). Similar to GENIUS, GPT4GNAS also use GPT-4 and give it a broad search search and use accuracy as the unique evaluation metric. Other than GPT4GNAS, DIFFNAS \cite{li2023diffnas} use LLMs to search neural architectures which are more compatible with Denoising Diffusion Probabilistic Models (DDPM). DIFFNAS , similarly to GENIUS and GPT4GNAS, maximizes the search space and includes all architecture parameters strongly related to Unet model, which is the base model of DDPM, in the search space. Other than applying in pure NAS, LCDA \cite{yan2023viability} explore the potential of utilizing LLMs in deploying neural architecture on edge devices which have stringent power and computational budget. Different from GENIUS, GPT4GNAS, and DIFFNAS, LCDA adds more constraints to the search space and confine the searchable neural architecture parameters within a small scope. This is because edge devices cannot hold large neural architectures and it is important to utilize available resources as efficiently as possible.

% With a clear understanding of the limitations inherent in conventional Neural Architecture Search (NAS) methods, there has been interest in implementing NAS in various novel ways. The emergence of Large Language Models (LLMs) presents an opportunity to accelerate the speed of neural architecture search and enhance the search performance. The currently most widely utilized advanced LLM is GPT-4 \cite{OpenAI2023GPT4TR}, which demonstrates superior logical inference capabilities across a range of professional \cite{bevilacqua2023automated} and academic benchmarks when compared to other existing language models such as Llama \cite{touvron2023llama}, Pythia \cite{biderman2023pythia}, and PaLM 2 \cite{anil2023palm}. Unlike classical transformer-based models \cite{devlin2018bert, liu2019roberta, sanh2019distilbert} and their related works \cite{qin2021ibert, luo2020open}, LLMs possess exponentially larger numbers of trainable parameters: Llama has 65B, GPT-3 has 175B, PaLM has 540B, and GPT-4 boasts 1.76T. Due to this vast number of trainable parameters, LLMs employ Mixture of Experts (MoEs) techniques \cite{artetxe2021efficient} and are trained on exceptionally large, high-quality datasets. For instance, Llama is trained on a dataset comprising CCNet [67\%], C4 [15\%], GitHub [4.5\%], Wikipedia [4.5\%], Books [4.5\%], ArXiv [2.5\%], and Stack Exchange [2\%] \cite{touvron2023llama}. All these factors endow LLMs with a broad domain knowledge, enabling the design and optimization of neural architectures for user-specific tasks.
With a clear understanding of the limitations inherent in conventional NAS methods, there has been interest in implementing NAS in various novel ways. The emergence of LLMs presents an opportunity to accelerate the speed of neural architecture search and enhance the search performance. The currently most widely utilized advanced LLM is GPT-4, which demonstrates superior logical inference capabilities across a range of professional \cite{bevilacqua2023automated} and academic benchmarks when compared to other existing language models such as Llama, Pythia, and PaLM-2. Unlike classical transformer-based DNNs such as BERT, RoBERTa, DistillBERT, and their related works \cite{qin2021ibert, luo2020open}, LLMs possess exponentially larger numbers of trainable parameters: Llama has 65B, GPT-3 has 175B, PaLM has 540B, and GPT-4 boasts 1.76T. Due to this vast number of trainable parameters, LLMs employ Mixture of Experts (MoEs) techniques and are trained on exceptionally large, high-quality datasets. For instance, Llama is trained on a dataset \cite{touvron2023llama} comprising CCNet [67\%], C4 [15\%], GitHub [4.5\%], Wikipedia [4.5\%], Books [4.5\%], ArXiv [2.5\%], and Stack Exchange [2\%]. All these factors endow LLMs with a broad domain knowledge, enabling the design and optimization of neural architectures for user-specific tasks.

GENIUS \cite{zheng2023can} is the pioneering work investigating the potential of utilizing GPT-4 for NAS. GENIUS employs GPT-4 as a "black box" with domain knowledge pertinent to neural architecture design. This "black box" is driven by prompts, which only provide GPT-4 with a broad and vague search scope, instructing it to focus solely on accuracy. Furthermore, GPT4GNAS \cite{wang2023graph} explores the potential of LLMs in Graph Neural Architecture Search (GNAS). Similar to GENIUS, GPT4GNAS also uses GPT-4, providing it with a broad search scope and using accuracy as the sole evaluation metric. In contrast, DIFFNAS \cite{li2023diffnas} employs LLMs to search for neural architectures that are more compatible with Denoising Diffusion Probabilistic Models (DDPM). Like GENIUS and GPT4GNAS, DIFFNAS maximizes the search space but includes all architecture parameters strongly related to the Unet model, which is the base model of DDPM, in the search space. Beyond pure NAS applications, LCDA \cite{yan2023viability} explores the potential of utilizing LLMs in deploying neural architectures on edge devices, which have stringent power and computational budgets. Unlike GENIUS, GPT4GNAS, and DIFFNAS, LCDA adds more constraints to the search space, confining the searchable neural architecture parameters within a narrower scope. This is necessitated by the fact that edge devices cannot accommodate large neural architectures, and it is crucial to utilize available resources as efficiently as possible.

% \subsection{\st{NAS via LLMs towards Fairness}}
\subsection{NAS via LLMs with Search Constraints}

% Fairness \cite{barocas2017fairness} attracts increasing attention as the development of machine learning models. While most models are evaluated by accuracy over the given data in general, the detailed difference among various groups in the given data is relatively ignored. Fairness can be understood as the difference between the same model performance in different groups with distinct demographic characteristics. With the increasing demand of deploying machine learning models on personalized devices, fairness is becoming a critical model evaluator. NAS, as an automatic model design framework, with the potential to design models to satisfy various situations on personalized devices, can be naturally compatible with fairness. 

Fairness in machine learning has garnered increasing attention with the proliferation of DNN. Unlike the conventional evaluation metric of accuracy across a given dataset, fairness delves into the nuanced performance differences among various demographic groups within the data. It essentially evaluates how a DNN performs across different groups characterized by distinct demographic attributes. As the deployment of DNN on personalized devices escalates, ensuring fairness has become a critical evaluation criterion. NAS, being an automated DNN design framework, holds the potential to tailor DNN to diverse scenarios on personalized devices, thereby aligning naturally with the ethos of fairness.
% \textcolor{blue}{yuting: As the integration of DNNs into personal devices becomes increasingly prevalent, the imperative of ensuring that the searched architectures of NAS adhere to constraints over performance and hardware specifications is paramount. For instance, ensuring fairness while keeping the model satisfied with hardware limitations is critical for some tasks running in different user-end devices.}


% FairNAS \cite{chu2021fairnas} introduces fairness to the NAS search constraints and systemically analyze the impact of NAS performance after having fiarness as the search constraint. Different from classical NAS frameworks depend on RNN controllers, FairNAS samples multiple models without replacement and train them sequentially. These models will be evaluated in parallel. Other than FairNAS, FNAS \cite{liu2021fnas} improve the fairness of searched models by sharing checkpoints in Architecture Knowledge Pool (AKP) and applying uncertainty functions. Later on, the concepts of NAS and fairness are extended into edge devices by FaHaNa \cite{sheng2022larger}, where fairness and hardware-limitations, along with the traditional model evaluator, overall accuracy, are used as the searching constraints. 

FairNAS \cite{chu2021fairnas} pioneers the integration of fairness into NAS search constraints, and systematically examines the impact on NAS performance post the inclusion of fairness as a search constraint. Unlike traditional NAS frameworks reliant on RNN controllers, FairNAS adopts a novel approach of sampling multiple DNN without replacement, and sequentially training them. These DNN are then evaluated in parallel. On a similar note, FNAS \cite{liu2021fnas} enhances the fairness of the resultant DNN by sharing checkpoints in the Architecture Knowledge Pool (AKP) and employing uncertainty functions. Extending the discourse of NAS and fairness to edge devices, FaHaNa \cite{sheng2022larger} incorporates fairness and hardware-limitations along with the conventional evaluation metric of overall accuracy, as search constraints.


\subsection{Evaluate DNN fairness}
By general concept, fairness can be understood such that the performances of the same DNN over different demographic groups are close and similar. The fairness score, in this way, can be calculated based on the accuracy difference between each demographic group and the overall accuracy. According to Sheng et al \cite{sheng2022larger}, the fairness gauges the bias across all demographic groups in a dataset. They introduce a metric named unfairness, measuring the performance discrepancy between individual groups and the overall dataset. Lower unfairness values indicate a fairer DNN.

The unfairness is computed as:
\begin{equation}
    \text{Unfairness} = \frac{1}{P} \sum_{j=1}^{P} | \text{Acc}_{j} - \text{Acc}_{\text{overall}} |
\end{equation}

where \( P \) is the total number of demographic groups, \( \text{Acc}_{j} \) is the accuracy of the \(j\)-th demographic group, \( \text{Acc}_{\text{overall}} \) is the overall accuracy across all demographic groups.

Additionally, equality of opportunity \cite{hardt2016equality}, as a widely used fairness metric, also addresses DNN discrimination. Unlike our unfairness score, which evaluates accuracy across demographic groups, Equality of Opportunity emphasizes fairness concerning positive samples. Under this metric, three sub-metrics exist: Equalized Odds (EODD), Equal Opportunity with respect to the positive class (EOPP1), and with respect to the negative class (EOPP2).
\begin{itemize}
    \item \textbf{Equalized Odds (EODD):} This sub-metric asserts that, given the same opportunity, the True Positive Rate (TPR) and False Positive Rate (FPR) should be consistent across all demographic groups. This measure aims to ensure fairness both in favorable and unfavorable outcomes.
    \item \textbf{Equal Opportunity with respect to the positive class (EOPP1):} Unlike EODD, EOPP1 solely focuses on the fairness in favorable outcomes. It considers a DNN fair when the TPR is consistent among all demographic groups, ensuring that each group has an equal opportunity in receiving positive outcomes.
    \item \textbf{Equal Opportunity with respect to the negative class (EOPP2):} Conversely, EOPP2 emphasizes fairness in unfavorable outcomes. It deems a DNN fair when the True Negative Rate (TNR) is consistent among all demographic groups, ensuring fairness in avoiding negative outcomes.
\end{itemize}

They can be calculated as the following:
\begin{equation}
    \text{EODD} = \frac{1}{P} \sum_{p=1}^{P} \max \left( \left| \frac{\text{TP}^{(1)}_{p}}{\text{P}^{(1)}_{p}} - \frac{\text{TP}^{(2)}_{p}}{\text{P}^{(2)}_{p}} \right|, \left| \frac{\text{FP}^{(1)}_{p}}{\text{N}^{(1)}_{p}} - \frac{\text{FP}^{(2)}_{p}}{\text{N}^{(2)}_{p}} \right| \right)
\end{equation}

\begin{equation}
    \text{EOPP1} = \frac{1}{P} \sum_{p=1}^{P} \left| \frac{\text{TP}^{(1)}_{p}}{\text{P}^{(1)}_{p}} - \frac{\text{TP}^{(2)}_{p}}{\text{P}^{(2)}_{p}} \right|
\end{equation}

\begin{equation}
    \text{EOPP2} = \frac{1}{P} \sum_{p=1}^{P} \left| \frac{\text{TN}^{(1)}_{p}}{\text{N}^{(1)}_{p}} - \frac{\text{TN}^{(2)}_{p}}{\text{N}^{(2)}_{p}} \right|
\end{equation}

% where $TP_p^{(1)}$ and $TP_p^{(2)}$ refer to the first group and second group in pair $p$, respectively

where \( P \) is the total number of demographic group pairs, \( \text{TP}_{p}^{(1)} \) and \( \text{TP}_{p}^{(2)} \) are the number of true positives for the first group and second group in pair \( p \), \( \text{FP}_{p}^{(1)} \) and \( \text{FP}_{p}^{(2)} \) is the number of false positives for the first group and second group in pair \( p \), \( \text{TN}_{p}^{(1)} \) and \( \text{TN}_{p}^{(2)} \) is the number of true negatives for the first group and second group in pair \( p \), and \( \text{N}_{p}^{(1)} \) and \( \text{N}_{p}^{(2)} \) is the total number of negative instances for the first group and second group in pair \( p \).

% where \( P \) is the total number of demographic group pairs, \( \text{TP}_{pi} \) is the number of true positives for group \( i \) in pair \( p \), \( \text{FP}_{pi} \) is the number of false positives for group \( i \) in pair \( p \), \( \text{TN}_{pi} \) is the number of true negatives for group \( i \) in pair \( p \), \( \text{P}_{pi} \) is the total number of positive instances for group \( i \) in pair \( p \), and \( \text{N}_{pi} \) is the total number of negative instances for group \( i \) in pair \( p \).

\subsection{Motivations}

% In the past works, we have witnessed the potential of NAS in autonomous model design. In particular, as the rising need of personalized machine learning models, the idea of NAS can be a competitive solution in dealing with various specific requirements. These requirements can be attributed into two main points: (1) The model performance in different users cannot be distinct, which is called fairness. (2) The model needs to satisfy the hardware limitations in memory space and computational power. While the existing works have not fully explore the possibility of adding fairness and hardware limitation as the NAS search constraints, the way to interpret these constraints into a simple way and execute them in NAS efficiently are also remain unstudied. With the rising of LLMs, their capability of understanding human-generated text enables us to investigate these issues. Hence, we propose a NAS framework backed by LLMs, where we can take the advantages of LLMs to enable the NAS framework efficiently find the appropriate neural architecture, which can be hardware-efficient, ensure the fairness without negatively impact the overall accuracy

In the past works, the prowess of NAS in autonomous DNN design has been duly noted, especially with the burgeoning demand for personalized DNN. NAS presents a competitive solution to address diverse specific requirements, which can be distilled into two focal points: (1) Ensuring uniform DNN performance across different users, a criterion known as fairness, and (2) Adhering to hardware constraints concerning memory space and computational power. While existing works have yet to fully explore the potential of incorporating fairness and hardware limitations as NAS search constraints, the elucidation and efficient execution of these constraints within NAS remain uncharted territories. With the advent of LLMs, their adeptness at comprehending human-generated text provides a springboard to delve into these issues. Consequently, we propose a NAS framework underpinned by LLMs, leveraging the strengths of LLMs to efficiently navigate the NAS framework towards identifying appropriate neural architecture that can meet specific constraints for different scenarios.
% \st{Such architectures are envisioned to be hardware-efficient, uphold fairness, and maintain high overall accuracy without compromise.}


% and  design personalized models. In 

% LLM -> NAS -> Hardware-efficient -> fairness

% \subsection{Lite neural architecture and its performance}

% What is lite neural architecture? simple structure, small size of trainable parameters

% Why do we need lite neural architecture? deploy it to user-end devices (limited memory space, limited power, limited computational resource, but do need high and equal performance across all users)

% lite neural architecture has disadvantages compare to large one: data sensitive, related to fairness

% \subsection{Neural architecture search and fairness}

% \subsection{Large Language models and prompt tuning}





==> 3_Proposed.tex <==
\section{Proposed FL-NAS Method}
\label{sec_method}

% \begin{algorithm}
% \caption{Constraints (\(Target\_ENVS\))}
% \label{alg:constraints}
% \begin{changemargin}{0.3cm}{0cm}  % Adjust the left margin as needed
% \begin{flushleft}
% // Input: \(Target\_ENVS\) contains the DNN running environment information \newline
% \textit{\textbf{\(\bm{Prompt_{constraints}}\)}} =
% \begin{itemize}
%     \item \textit{The lower the unfairness score, the fairer the DNN. During search, you should increase your generated DNN accuracy and lower unfairness score}
%     \item \textit{You can explore different depths of DNN, but you need to consider the possibility of deploying DNN on \(Target\_ENVS[device\; name]\) with limited computing resources: \(Target\_ENVS[memory]\), \(Target\_ENVS[computation\; resource]\)}
%     \item \textit{Your neural architecture should have low latency, low throughput, and use as much less memory as possible}
%     \item \textit{You should try different normalization methods, different activation functions, and different pooling methods}
%     \item \textit{For these methods, functions, and convolutional layers, you should try different kernel size, filter size}
% \end{itemize}
% \end{flushleft}
% \end{changemargin}
% \end{algorithm}

\subsection{Framework Overview}




This paper proposes a framework to utilize LLM to efficiently search for DNN architecture in terms of fairness. Each searched architecture will be evaluated based on hardware efficiency and learning efficiency including accuracy and fairness. We leverage each evaluation metric and enable this framework to improve DNN fairness without negatively impact the other metrics. We name this framework as \textbf{F}airness utilizing \textbf{L}arge Language Models on \textbf{N}eural \textbf{A}rchitecture \textbf{S}earch.

For the sake of evaluation consistency, we choose a widely used dermatological dataset ISIC \cite{isic2019}. The people can be classified into young which is under 30, middle age which is under 65, and old which is above 65. The people in this dataset can also be classified based on biological gender which is female and male.

As shown in Algorithm ~\ref{alg:FLNAS}, the proposed framework takes the proper DNN template \textit{Template} the DNN deployment environment \textit{Target\_Evns}, the number of search iterations \textit{Search\_max}, and searching space \textit{Choices} as the input, and produce the DNN architecture \textit{Best\_DNN\_arch} with the best evaluation \textit{Best\_DNN\_eval} as the output. FLNAS consists of three components: (1) Design Optimizer, (2) Design Generator, (3) DNN Evaluator.


% In this section, we present FLNAS, our novel framework improving \textbf{F}airness utilizing \textbf{L}arge Language Models on \textbf{N}eural \textbf{A}rchitecture \textbf{S}earch. FLNAS can consider the limited resources and seeks to design a neural architecture that can run on the limited resources with high performance across all users and high fairness to all users from different demographic backgrounds. FLNAS comprises three core components: (1) LLM controller, (2) greedy neural architecture searching strategy (greedy strategy), and (3) neural architecture bank


\begin{algorithm}[t!]
\footnotesize
\caption{FLNAS Algorithm}\label{alg:FLNAS}
\begin{algorithmic}[1]

\State \textbf{Input:} Template, Target\_Envs, Search\_max, Choices
\State \textbf{Output:} $BestDNN_{arch}$, $BestDNN_{eval}$

\State Initialize $M_{arch}$ // A dictionary, where one name corresponds to one DNN architecture
\State Initialize $M_{eval}$ // A dictionary, where one name corresponds to one performance of that DNN architecture
\State // BestEvaluation is a function to get the best fairness performance and best accuracy 
\For{$i \gets 1$ \textbf{to} Search\_max}
    \State $DNN_{name} \gets$ BestEvaluation($M_{eval}$)
    \State $DNN_{arch} \gets M_{arch}[DNN_{name}]$
    \State $eval$ = $M_{eval}[DNN\_name]$ 
    \State $Prompt \gets$ PromptGenerator($DNN\_arch$, $eval$, $Template$, $Target_{Envs}$, $Choice$)
    \State $DNN_{arch}, DNN_{name} \gets$ LLM($Prompt$)
    \State $DNN_{eval} \gets$ DNN\_Evaluator($DNN_{arch}$)
    \State $M_{arch}[DNN_{name}] \gets DNN_{arch}$
    \State $M_{eval}[DNN_{name}] \gets DNN_{eval}$
\EndFor
\State $DNN_{name} \gets$ BestEvaluation($M_{eval}$)
\State $BestDNN_{eval} \gets$ $M_{eval}[DNN_{name}]$
\State $BestDNN_{arch} \gets$ $M_{arch}[DNN_{name}]$

\State \Return $BestDNN_{arch}$, $BestDNN_{eval}$

\end{algorithmic}
\end{algorithm}


% \begin{algorithm}
% \small
% \caption{FLNAS(\(Target\_ENVS, Template, Epoch_{max}\))}
% \label{alg:flnas}
% \begin{changemargin}{0.3cm}{0cm}
% //Input: \(Template\) gives LLMs a neural architecture format. \(Target\_ENVS\) contains the running environment information. \(Epoch_{max}\) indicates the max search \newline
% Initialize \(M_d, M_p\) \newline
% Initialize \(constraints_i\) = Constraints(\(Target\_ENVS\)) \newline
% \textbf{for} i in range(\(Epoch_{max}\)) \textbf{do} 
%     \begin{changemargin}{0.3cm}{0cm}
%         \(prompt\) = Prompt-Generator(\(M_d, M_p,\) $constraints_i$, Template) \newline
%         \(LLM\_response\) = \(prompt \rightarrow LLM\) \newline
%         \(DNN\) = \(LLM\_response \rightarrow extract\_DNN\) \newline
%         % Initialize \(Perf\_dict, val\_loss\) \newline
%         % // \(Perf\_dict\) is to track model detailed performance in each training iteration \newline
%         \(M_d[DNN\_name] \leftarrow DNN\) \newline
%         \textbf{for} j in range(training iterations) \textbf{do}
%         \begin{changemargin}{0.3cm}{0cm}
%             Get DNN performance: \(acc_t, loss_t, acc_v, loss_v\), \{\(acc_{vf}\) for $f$ in group\} \newline
%             Get hardware evaluation \newline
%             \textbf{if} satisfy early stop by validation loss
%             \begin{changemargin}{0.3cm}{0cm}
%                 \(unfairness\_score\) = \textit{Fairness-Score(Data, $Data_{group}$, DNN)}
%                 \(M_p[DNN\_name] \leftarrow\) all performance and evaluation
%             \end{changemargin}
%             % \textbf{end if}
%         \end{changemargin}
%         % \textbf{end for}
%     \end{changemargin}
%     % \textbf{end for}
% \end{changemargin}
% \end{algorithm} 


\subsection{LLM Optimizer}

The LLM optimizer serves as a pivotal component in FLNAS. It analyzes the searched best-performing DNN architecture and revised the architecture based on certain constraints. Existing methods using reinforcement learning or genetic algorithms, while demonstrating effectiveness in the searched DNN architecture, can take hundreds of GPU hours and hundreds of computational resources. This is because the existing methods mostly have a ``cold start" and they need numerous iterations to approach the appropriate answer without consider the heuristic knowledge that could largely accelerate the searching process.

In LLM optimizer, where it can utilize the knowledge trained on extensive human language corpora,  can circumvent the ``cold start" and trivial iteration issues to generate and optimize DNN architecture with less computational resources. To do that, there are two things the LLM optimizer need: (1) Searched Architectures and their evaluations and (2) Prompt Generator.

As shown in Algorithm ~\ref{alg:FLNAS}, searched architecture \textit{M\_arch} and their evaluations \textit{M\_eval} are initialized when FLNAS search for DNN architectures. Each searched DNN architecture will be assigned an unique name and used as key to access the saved architectures and evaluations. LLM optimizer will always use architecture with best evaluation to revise and design the new architecture. In this way, the LLM can also optimize from the best-performing architecture.

Prompt generator shown in Algorithm ~\ref{alg:FLNAS} as ``PromptGenerator'', where it generates a prompt containing necessary information to design DNN. It takes the current best performed DNN architecture \textit{DNN\_arch}, that DNN evaluation \textit{eval}, the proper DNN format \textit{Template} which can be parsed and executed properly, the number of searches can make \textit{Search\_max}, and the available kernel sizes can choice \textit{Choices}. As shown in Algorithm ~\ref{alg:prompt-generator}, the prompt generator contains two main parts. The first part is about DNN related information including its architecture, its evaluation, and its deployment environment. The second part is about searching constraints, where the different importance level of metrics are explained and the available searching space is defined.

% LLM controller serves as a crucial component in FLNAS framework. It analyze the current searched best performed model and revise the model based on given search constraints described in Algorithm ~\ref{alg:constraints}. LLM controller is designed to take the place of RNN controller widely used in classical NAS frameworks. The core component in LLM controller is a LLM, which can be a local LLM for data security and privacy issues or a LLM api for computational power efficiency and obtaining the fully inference power of LLM. In this work, we choose GPT-4 api \cite{OpenAI2023GPT4TR} as the LLM component due to targeting the resource efficiency. 
% The LLM Optimizer acts as a pivotal component within the FLNAS framework. It analyzes the currently searched best-performing DNN and revises the DNN based on the given search constraints as described in Algorithm ~\ref{alg:constraints}. The LLM Optimizer is designed to replace the RNN controller commonly utilized in traditional NAS frameworks. At the heart of the LLM Optimizer is a Language Model, which can either be a local Language Model addressing data security and privacy concerns, or a Language Model API, which is preferred for computational efficiency and to leverage the full inference power of the Language Model. In this work, we opt for the GPT-4 API \cite{OpenAI2023GPT4TR} as the LLM component, targeting resource efficiency.
\begin{algorithm}
\caption{PromptGenerator(arch, eval, Template, Target\_Envs, Choices)}
\footnotesize
\label{alg:prompt-generator}
\begin{changemargin}{0.3cm}{0cm}
\begin{flushleft}
//Input: arch: current architecture, eval: current evaluation, Template: neural architecture format, Target\_Envs: deployment environment, Choices: available choices for modification \newline
\textit{\textbf{\(\bm{Prompt_{s}}\)} = ``You are an expert in the field of neural architecture search.''} \newline
\textit{\textbf{\(\bm{Prompt_{code}}\)} = ``You need to follow the format in \{Template\} to generate a DNN architecture''} \newline
\textit{\textbf{\(\bm{Prompt_{u}}\)}} = ``Your task is to design a DNN architecture to process the image from ISIC dataset for image classification task. The current best-performing DNN architecture is \{arch\} and its evaluation is \{eval\}. 

Your designed DNN will be deployed into \{Target\_Envs\}, so you need to make sure you consider the limitations in this running environment.

In evaluation, the metrics are accuracy, fairness, and hardware efficiency. You need to Improve the fairness without decreasing the accuracy. Also notice the accuracy in each demographic group and the overall accuracy. Try to design a DNN to improve the lowest accuracy in certain demographic groups.

Regarding the hardware efficiency metrics, which are number of parameters, latency, and memory, you should try to minimize them so the DNN can run with less resources. But the priority of optimizing hardware efficiency is lower than maintaining high accuracy, which is also lower than improving fairness.

You can insert or remove convolutional layers, use different normalization methods, regularization methods, and try different sizes of kernel. The available range is \{Choices\}
''

return \textbf{\(\bm{Prompt_{s}}\)} + \textbf{\(\bm{Prompt_{code}}\)} + \textbf{\(\bm{Prompt_{u}}\)}
\end{flushleft} 
\end{changemargin}
\end{algorithm}

% \begin{algorithm}
% \caption{Prompt-Gen(\(M_{d}\), \(M_{p}\), \(Contraints\), \(Template\))}
% \small
% \label{alg:prompt-generator}
% \begin{changemargin}{0.3cm}{0cm}
% \begin{flushleft}
% //Input: \(M_{d}\): \(\{<DNN\; name>: <DNN\; structure>\}\),  \(M_{p}\): \(\{<DNN\; name>: <DNN\; performance>\}\), \(Constraints\): \textit{search space}, \(Template\): \textit{neural architecture format} \newline
% \( M_p \rightarrow M_{best}(Accuracy_{max}, Unfairness_{min})\) \newline
% % \( M_{d}[M_(best)] \rightarrow \) best neural architecture \newline
% \( M_{p}[M_{best}] \rightarrow Performance\; detail \) \newline
% \textit{\textbf{\(\bm{Prompt_{s}}\)} = "Your task is to design a CNN architecture for skin cancer classification, while considering the fairness and computational resource efficiency"} \newline
% \textit{\textbf{\(\bm{Prompt_{u1}}\)} = "You need to follow this template to design your neural architecture: {\(Template\)}"} \newline
% \textit{\textbf{\(\bm{Prompt_{u2}}\)} = "Your code need always include 'import torch.nn as nn' and 'import torch'"}
% \begin{itemize}
%     \item \textit{Your code format should also satisfy the following:}
%     \begin{itemize}
%         \item \textit{This neural architecture should handle 2D images.}
%         \item \textit{You can add, cut, or modify convolutional layers, but make sure the conv layers input and output have the correct shape.}
%         \item \textit{Use Dummy Test to get correct final output shape}
%         \item \textit{In the forward function, add \(x.view(-1, self.flattened\_size)\) and \(self.fc(x)\) in the very end.}
%         \item \textit{Provide the pytorch complete code in your response, also include \(import \: torch.nn \: as \: nn\).}
%         \item \textit{You need to have the \( \text{num\_classes} \) as the only parameter in the \( \_\_init\_\_ \) function.}
%     \end{itemize}
%     \item \textit{The current best neural architecture is \(M_{best}\), its performance is \(M_{p}[M_{best}]\).}
%     \item \textit{To optimize the neural architecture, you need to consider the following constraints: \{constraints\}}
% \end{itemize}
% return \textbf{\(\bm{Prompt_{s}}\)} + \textbf{\(\bm{Prompt_{u1}}\)} + \textbf{\(\bm{Prompt_{u2}}\)}
% \end{flushleft} 
% \end{changemargin}
% \end{algorithm}

% To drive GPT-4, a prompt-generator, described in Algorithm ~\ref{alg:prompt-generator} is required. There are three components in the prompt-generator: (1) the neural architecture and detailed performance of the best model, (2) respond neural architecture format, and (3) search constraints regarding search space. LLM is necessary to know the neural architecture of the best model in order to revise its structure. For the detailed performance, instead of only feeding the model overall accuracy to LLM, we provide the model accuracy on every demographic group and the sample size, the unfairness score, and equality of opportunity metrics, which will be elaborated in the later section, to LLM. Here is an example of detailed performance: \textit{Train Loss: $0.8746$, Train Acc: $58.06\%$, Valid Loss: $0.6438$, Valid Acc: $62.80\%$, unfairness Score: $1.2983$, EODD: $0.1229$, EOPP1: $0.1224$, EOPP2: $0.0105$, Fairness Detail: [male: ($63.23\%$, $95$), female: ($62.37\%$, $93$), young: ($25.99\%$, $23$), middle\_age: ($59.30\%$, $104$), old: ($81.82\%$, $62$)] Latency: $0.002153$ seconds per image, Throughput: $464.38$ images per second, Peak GPU Memory Usage: $232.88$ MB}
% To operate GPT-4, a prompt-generator, delineated in Algorithm ~\ref{alg:prompt-generator}, is essential. The prompt-generator comprises three components: (1) the neural architecture and detailed performance of the best DNN, (2) the response neural architecture format, and (3) search constraints concerning the search space. It is imperative for the LLM to comprehend the neural architecture of the best DNN to aptly revise its structure. Rather than merely supplying the overall DNN accuracy to the LLM, we furnish accuracy details for every demographic group along with sample size, the unfairness score, and equality of opportunity metrics (elaborated in a subsequent section) to the LLM. 

As we explained, the DNN evaluation will be fed into LLM. Instead of only provide a single value, which is less informative, we provide a detailed evaluation, where every demographic group evaluation and the hardware evaluation are provided LLM a comprehensive understanding of the DNN evaluation. The following is an example of detailed performance: \textit{Train Loss: $0.8746$, Train Acc: $58.06\%$, Valid Loss: $0.6438$, Valid Acc: $62.80\%$, Unfairness Score: $1.2983$, EODD: $0.1229$, EOPP1: $0.1224$, EOPP2: $0.0105$, Fairness Detail: [male: ($63.23\%$, $95$), female: ($62.37\%$, $93$), young: ($25.99\%$, $23$), middle\_age: ($59.30\%$, $104$), old: ($81.82\%$, $62$)] Latency: $0.002153$ seconds per image, Throughput: $464.38$ images per second, Peak GPU Memory Usage: $232.88$ MB}.

% \begin{algorithm}
% \caption{Constraints (\(Target\_ENVS\))}
% \label{alg:constraints}
% \begin{changemargin}{0.3cm}{0cm}  % Adjust the left margin as needed
% \begin{flushleft}
% // Input: \(Target\_ENVS\) contains DNN environment info. \newline
% \textit{\textbf{\(\bm{Prompt_{constraints}}\)}} =
% \begin{itemize}
%     \item Optimize for higher DNN accuracy and lower unfairness score.
%     \item Consider DNN depth and deployment on \(Target\_ENVS[device\; name]\) with resources: \(Target\_ENVS[memory]\), \(Target\_ENVS[comp.\; resource]\).
%     \item Aim for low latency, throughput, and memory usage.
%     \item Explore different normalization, activation functions, and pooling methods.
%     \item Experiment with kernel and filter sizes for layers and methods.
% \end{itemize}
% \end{flushleft}
% \end{changemargin}
% \end{algorithm}

% \begin{algorithm}
% \caption{Constraints (\(Target\_ENVS\))}
% \small
% \label{alg:constraints}
% \begin{changemargin}{0.3cm}{0cm}  % Adjust the left margin as needed
% \begin{flushleft}
% // Input: \(Target\_ENVS\) contains the DNN running environment information \newline
% \textit{\textbf{\(\bm{Prompt_{constraints}}\)}} =
% \begin{itemize}
%     \item \textit{The lower the unfairness score, the fairer the DNN. During search, you should increase your generated DNN accuracy and lower unfairness score}
%     \item \textit{You can explore different depths of DNN, but you need to consider the possibility of deploying DNN on \(Target\_ENVS[device\; name]\) with limited computing resources: \(Target\_ENVS[memory]\), \(Target\_ENVS[computation\; resource]\)}
%     \item \textit{Your neural architecture should have low latency, low throughput, and use as much less memory as possible}
%     \item \textit{You should try different normalization methods, different activation functions, and different pooling methods}
%     \item \textit{For these methods, functions, and convolutional layers, you should try different kernel size, filter size}
% \end{itemize}
% \end{flushleft}
% \end{changemargin}
% \end{algorithm}

% Due to the uncertainty of LLM response, the searched neural architecture may not be always the same format and executable. Hence, to make sure the search can be continuously processed, it is important to provide a strict response format for LLM to follow.
% Due to the unpredictable nature of the LLM response, the searched neural architecture may not always conform to the same format and be executable. Hence, providing a stringent response format for the LLM to adhere to is pivotal to ensure the continuous processing of the search.


% Search constraints define the search space. Different from existing NAS frameworks, FLNAS does not provide a specific range or specific parameter values to search. For NAS frameworks reply on RNN controller, the implicit search space can lead to overwhelming computation cost and lower the possibility of finding the optimal neural architecture. We argue that given a specific search space can confine the FLNAS capability of find the optimal neural architecture in edge cases when the ideal model should be very large or very small. Instead, we concentrate on the high-level performance. With the detailed performance, we ask the LLM to find a neural architecture with higher accuracy and lower unfairness score.
% Search constraints delineate the search space. Unlike existing NAS frameworks, FLNAS does not specify a particular range or parameter values for the search. For NAS frameworks reliant on the RNN controller, the implicit search space could escalate computational costs and diminish the likelihood of discovering the optimal neural architecture. We contend that specifying a search space might constrain FLNAS's ability to unearth the optimal neural architecture in edge cases, especially when the ideal DNN should be exceedingly large or small. Instead, we focus on high-level performance. Armed with detailed performance data, we task the LLM with finding a neural architecture that boasts higher accuracy and a lower unfairness score.

% \begin{algorithm}
% \small
% \caption{FLNAS(\(Target\_ENVS, Template, Epoch_{max}\))}
% \label{alg:flnas}
% \begin{changemargin}{0.3cm}{0cm}
% //Input: \(Template\) gives LLMs a neural architecture format. \(Target\_ENVS\) contains the running environment information. \(Epoch_{max}\) indicates the max search \newline
% Initialize \(M_d, M_p\) \newline
% Initialize \(constraints_i\) = Constraints(\(Target\_ENVS\)) \newline
% \textbf{for} i in range(\(Epoch_{max}\)) \textbf{do} 
%     \begin{changemargin}{0.3cm}{0cm}
%         \(prompt\) = Prompt-Generator(\(M_d, M_p,\) $constraints_i$, Template) \newline
%         \(LLM\_response\) = \(prompt \rightarrow LLM\) \newline
%         \(DNN\) = \(LLM\_response \rightarrow extract\_DNN\) \newline
%         % Initialize \(Perf\_dict, val\_loss\) \newline
%         % // \(Perf\_dict\) is to track model detailed performance in each training iteration \newline
%         \(M_d[DNN\_name] \leftarrow DNN\) \newline
%         \textbf{for} j in range(training iterations) \textbf{do}
%         \begin{changemargin}{0.3cm}{0cm}
%             Get DNN performance: \(acc_t, loss_t, acc_v, loss_v\), \{\(acc_{vf}\) for $f$ in group\} \newline
%             Get hardware evaluation \newline
%             \textbf{if} satisfy early stop by validation loss
%             \begin{changemargin}{0.3cm}{0cm}
%                 \(unfairness\_score\) = \textit{Fairness-Score(Data, $Data_{group}$, DNN)}
%                 \(M_p[DNN\_name] \leftarrow\) all performance and evaluation
%             \end{changemargin}
%             % \textbf{end if}
%         \end{changemargin}
%         % \textbf{end for}
%     \end{changemargin}
%     % \textbf{end for}
% \end{changemargin}
% \end{algorithm} 


\subsection{Designer Generator}
The designer generator will takes the LLM output and check whether the output contains valid DNN architecture, where the input and output of each convolutional layers can be processed properly. 
If it identifies an invalid DNN architecture, it will ask LLM to regenerate until a valid DNN architecture is detected. The LLM generated DNN architecture is shown in Fig. ~\ref{fig:example}. Then, DNN architecture will be parsed into executable DNN model.

\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{example.png}
  % \caption{Micro-Controller guides data selector and uses the three-step evaluator to update the data loader in data selector. }
  \caption{LLM response example}
  \label{fig:example}
\end{figure}
% \subsection{Greedy strategy}

\subsection{DNN Evaluator}

The DNN evaluator is designed to evaluate the DNN architecture made by LLM. It shown as \textit{Evaluate()} in Algorithm ~\ref{alg:FLNAS}. The DNN evaluator evaluate the DNN in two levels: the DNN itself and its hardware efficiency. Given a DNN, it will train the DNN with same hyperparameter settings and stop the training when validation loss no longer decreases. The train accuracy, train loss, validation accuracy, and validation loss at that epoch step will be kept. Meanwhile, the individual accuracy of each demographic group is also simultaneously calculated, along with the EODD, EOPP1, and EOPP2. For the hardware efficiency, we record inference latency, trainable parameters in the DNN, and storage memory required to save the DNN model. All of these stats will be maintained and integrated as the evaluation of the DNN.

% Model: Accuracy, Fairness, EODD, EOPP1, EOPP2

% Hardware: Latency, Memory, number of paramters

% When design the prompt generator, we only give the LLM the best performed model information and directly ask LLM to revise and improve the best performed model. Compared to LLM-based NAS work like LCDA \cite{yan2023viability}, which provides all searched model information, our strategy makes the LLM always concentrates on the best performed model, so we named our strategy as greedy strategy. As the prompt tuning research \cite{lester2021power} states, LLM can better understand and generate effective response when being given concise and lite prompts. We argue that provides all searched model information can be redundant and decrease the LLM decision-making capability. 
% In designing the prompt generator, we exclusively furnish the LLM with the best-performing DNN's information, directly urging the LLM to revise and enhance the best-performing DNN. Contrary to LLM-based NAS work like LCDA \cite{yan2023viability}, which supplies all searched DNN information, our strategy keeps the LLM focused solely on the best-performing DNN, hence we dub our strategy as the ``greedy strategy.'' As the research on prompt tuning suggests \cite{lester2021power}, LLM can better comprehend and generate effective responses when provided with concise and streamlined prompts. We argue that presenting all searched DNN information could be superfluous and potentially impair the LLM's decision-making capability.


% \subsection{Neural architecture bank}

% % As Algoirhtm ~\ref{alg:prompt-generator} described, we have $M_d$ and $M_p$ to keep track of the searched neural architectures and their performances. Neural architecture bank consists of $M_d$ and $M_p$, where both keys are the model names. While we only provide the best neural architecture and its performance during each prompt generating, we still keep track the searching history. After FLNAS finishes amount of search iterations defined by users, we can select the best performed neural architecture from $M_d$ and $M_p$.
% As Algorithm ~\ref{alg:prompt-generator} outlines, we employ $M_d$ and $M_p$ to keep a record of the searched neural architectures and their performances. The Neural Architecture Bank comprises $M_d$ and $M_p$, where both keys represent the DNN names. Although we only provide the best neural architecture and its performance during each prompt generation, we still maintain a history of the search. Upon the completion of a user-specified number of search iterations, we can select the best-performing neural architecture from $M_d$ and $M_p$.


% \subsection{Framework Overview}

% % The FLNAS framework explores the optimal neural architecture design based on greedy strategy up to a user-specified search iterations. In each iteration, the prompt is automatically generated based by Algorithm ~\ref{alg:prompt-generator}, with the search space defined by Algorithm ~\ref{alg:constraints}. The output of Algorithm ~\ref{alg:prompt-generator} will be parsed into executable model and evaluated based on metrics described in section 4.2. After finish neural architecture search, we can get two dictionary storing all searched model architectures and performances, where we can select the best performed models.
% The FLNAS framework endeavors to explore the optimal neural architecture design based on the greedy strategy up to a user-specified number of search iterations. In each iteration, the prompt is autonomously generated by Algorithm ~\ref{alg:prompt-generator}, with the search space defined by Algorithm ~\ref{alg:constraints}. The output of Algorithm ~\ref{alg:prompt-generator} is parsed into an executable DNN and evaluated based on the metrics described in Section 4.2. Upon concluding the neural architecture search, we obtain two dictionaries storing all searched DNN architectures and performances, from which we can select the best-performing DNN.


% [Have a short overview]

% Let's name is as LLMnas for now.

% \subsection{LLM Controller}

% \subsection{Neural Architecture Bank}

% \subsection{Neural Architecture Performance Evaluator}
% \subsubsection{Accuracy and fairness score}
% \subsubsection{Latency, storage, and parameter size}

% \subsection{Framework Overview}

==> 4_Experiment.tex <==
\section{Experimental Evaluation}
\label{sec_exp}

\captionsetup[table]{skip=4pt}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}


% \begin{table*}[t]
% \centering
% \caption{Comparison of classical DNN and FLNAS searched DNNs}
% \label{tab:evaluation}
% \begin{tabular}{c|c|P{1.7cm}P{1.7cm}P{1.8cm}P{1.5cm}|P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}}
% \toprule
% \midrule
% \multicolumn{2}{c|}{\multirow{2}{*}{DNN}} & \multicolumn{4}{c|}{\textbf{Hardware Efficiency Evaluation}} & \multicolumn{5}{c}{\textbf{DNN Evaluation}} \\
% \multicolumn{2}{c|}{} & \# of Para. & Latency (ms) Nvidia A10 & Latency (ms) Raspberry Pi 4 & Mem (MB) & accuracy & unfairness & EODD & EOPP1 & EOPP2 \\
% \midrule
% \multirow{5}{*}{\rotatebox{90}{Baseline}} & ResNet-18 & 11,169,858 & 0.763 & 5.64 & 2113.91 & 66.67\% & 0.3200 & 0.1077 & 0.0726 & 0.1006 \\
% & ResNet-34 & 21,278,018 & 1.450 & 11.26 & 3503.10 & 63.80\% & 0.4354 & 0.1556 & 0.0856 & 0.1335 \\
% & MobileNetV1 & 3,199,106  & 0.594 & 1.31 & 1108.89 & 67.73\% & 0.3498 & 0.1470 & 0.0482 & 0.1287 \\
% & MobileNetV2 & 7,054,850  & 1.563 & 1.62 & 2444.69 & 66.93\% & 0.5778 & 0.1697 & 0.0445 & 0.1620 \\
% & FaHaNa-Fair & 5,532,866  & 0.644 & 3.42 & 12864.62 & 71.73\% & 0.2570 & 0.1247 & 0.0583 & 0.1155 \\
% \midrule
% \multirow{3}{*}{\rotatebox{90}{FLNAS}} & Search-1  & $  $3,309,570  & $ \downarrow $0.273 & $\downarrow$0.11 & $ \downarrow $211.79  & $ \uparrow $75.20\% & $ \downarrow $0.1044 & $  $0.1711 & $ \downarrow $0.0346 & $  $0.1711 \\
% & \textbf{Search-2}  & $ \downarrow $\textbf{293,954} & $ \downarrow $\textbf{0.155} & $\downarrow$\textbf{0.15} & $ \downarrow $\textbf{232.88}  & $ \uparrow $\textbf{73.20\%} & $ \downarrow $\textbf{0.0306} & $ \downarrow $\textbf{0.0995} & $ \downarrow $\textbf{0.0340} & $ \downarrow $\textbf{0.0995} \\
% & Search-3  & $ \downarrow $148,098    & $ \downarrow $0.241 & $\downarrow$0.08 & $ \downarrow $158.25  & $ \uparrow $72.00\% & $ \downarrow $0.1136 & $  $0.1107 & $ \downarrow $0.0204 & $  $0.1107 \\
% \midrule
% \multicolumn{11}{l}{\footnotesize \textbf{Note:} "Arrow" indicates FLNAS improves (increases or reduces) the corresponding metric value compared to all baselines.} \\
% \midrule
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{Comparison of classical DNN and FLNAS searched DNNs}
% \label{tab:evaluation}
% \begin{tabular}{c|c|P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}|P{1.7cm}P{1.7cm}|P{1.8cm}P{1.5cm}}
% \toprule
% \midrule
% \multicolumn{2}{c|}{\multirow{2}{*}{DNN}} & \multicolumn{5}{c|}{\textbf{DNN Evaluation}} & \multicolumn{2}{c|}{\textbf{Latency (ms)}} & \multicolumn{2}{c}{\textbf{Hardware Efficiency}} \\
% \multicolumn{2}{c|}{} & Accuracy & Unfairness & EODD & EOPP1 & EOPP2 & Nvidia A10 & Raspberry Pi 4 & \# of Para. & Mem (MB) \\
% \midrule
% \multirow{5}{*}{\rotatebox{90}{Baseline}} 
% & ResNet-18 & 66.67\% & 0.3200 & 0.1077 & 0.0726 & 0.1006 & 0.763 & 5.64 & 11,169,858 & 2113.91 \\
% & ResNet-34 & 63.80\% & 0.4354 & 0.1556 & 0.0856 & 0.1335 & 1.450 & 11.26 & 21,278,018 & 3503.10 \\
% & MobileNetV1 & 67.73\% & 0.3498 & 0.1470 & 0.0482 & 0.1287 & 0.594 & 1.31 & 3,199,106 & 1108.89 \\
% & MobileNetV2 & 66.93\% & 0.5778 & 0.1697 & 0.0445 & 0.1620 & 1.563 & 1.62 & 7,054,850 & 2444.69 \\
% & FaHaNa-Fair & 71.73\% & 0.2570 & 0.1247 & 0.0583 & 0.1155 & 0.644 & 3.42 & 5,532,866 & 12864.62 \\
% \midrule
% \multirow{3}{*}{\rotatebox{90}{FLNAS}} 
% & Search-1 & 75.20\% & 0.1044 & 0.1711 & 0.0346 & 0.1711 & 0.273 & 0.11 & 3,309,570 & 211.79 \\
% & \textbf{Search-2} & \textbf{73.20\%} & \textbf{0.0306} & \textbf{0.0995} & \textbf{0.0340} & \textbf{0.0995} & \textbf{0.155} & \textbf{0.15} & \textbf{293,954} & \textbf{232.88} \\
% & Search-3 & 72.00\% & 0.1136 & 0.1107 & 0.0204 & 0.1107 & 0.241 & 0.08 & 148,098 & 158.25 \\
% \midrule
% \multicolumn{11}{l}{\footnotesize \textbf{Note:} "Arrow" indicates FLNAS improves (increases or reduces) the corresponding metric value compared to all baselines.} \\
% \midrule
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[t]
\centering
\caption{Comparison of classical DNN and FLNAS searched DNNs}
\label{tab:evaluation}
\begin{tabular}{c|c|P{1.1cm}P{1.1cm}P{1.1cm}P{1.1cm}P{1.1cm}|P{1.3cm}P{1.4cm}|P{1.4cm}P{1.9cm}}
\toprule
\midrule
\multicolumn{2}{c|}{\multirow{2}{*}{DNN}} & \multicolumn{5}{c|}{\textbf{DNN Evaluation}} & \multicolumn{2}{c|}{\textbf{Hardware Efficiency}} & \multicolumn{2}{c}{\textbf{Latency (s)}} \\
\multicolumn{2}{c|}{} & Accuracy & Unfairness & EODD & EOPP1 & EOPP2 & \# of Para. & Mem (MB) & Nvidia A10 & Raspberry Pi 4 \\
\midrule
\multirow{5}{*}{\rotatebox{90}{Baseline}} 
& ResNet-18 & 66.67\% & 0.3200 & 0.1077 & 0.0726 & 0.1006 & 11,169,858 & 2113.91 & 0.00763 & 5.64 \\
& ResNet-34 & 63.80\% & 0.4354 & 0.1556 & 0.0856 & 0.1335 & 21,278,018 & 3503.10 & 0.01450 & 11.26 \\
& MobileNetV1 & 67.73\% & 0.3498 & 0.1470 & 0.0482 & 0.1287 & 3,199,106 & 1108.89 & 0.00594 & 1.31 \\
& MobileNetV2 & 66.93\% & 0.5778 & 0.1697 & 0.0445 & 0.1620 & 7,054,850 & 2444.69 & 0.01563 & 1.62 \\
& FaHaNa-Fair & 71.73\% & 0.2570 & 0.1247 & 0.0583 & 0.1155 & 5,532,866 & 12864.62 & 0.00644 & 3.42 \\
\midrule
\multirow{3}{*}{\rotatebox{90}{FLNAS}} 
& Search-1 & \textuparrow 75.20\% & \textdownarrow 0.1044 & 0.1711 & \textdownarrow 0.0346 & 0.1711 & \textdownarrow 3,309,570 & \textdownarrow 211.79 & \textdownarrow 0.00273 & \textdownarrow 0.11 \\
& \textbf{Search-2} & \textuparrow \textbf{73.20\%} & \textdownarrow \textbf{0.0306} & \textdownarrow \textbf{0.0995} & \textdownarrow \textbf{0.0340} & \textdownarrow \textbf{0.0995} & \textdownarrow \textbf{293,954} & \textdownarrow \textbf{232.88} & \textdownarrow \textbf{0.0011} & \textdownarrow \textbf{0.15} \\
& Search-3 & \textuparrow 72.00\% & \textdownarrow 0.1136 & 0.1107 & \textdownarrow 0.0204 & 0.1107 & \textdownarrow 148,098 & \textdownarrow 158.25 & \textdownarrow 0.00241 & \textdownarrow 0.08 \\
\midrule
\multicolumn{11}{l}{\footnotesize \textbf{Note:} ``Arrow" indicates FLNAS improves (increases or reduces) the corresponding metric value compared to all baselines.} \\
\midrule
\bottomrule
\end{tabular}
\end{table*}


\subsection{Experimental Setup}
We design experiments to demonstrate the superior performance of FLNAS in given image classification tasks. We compare FLNAS with other popular DNNs under the same settings. We use one Nvidia A10 as the engine to evaluate the LLM searched DNN architecture. For the searched architecture, we also examine their inference latency in Raspberry Pi 4.

% \textit{\textbf{A. Dataset:}} We use a classical dataset from ISIC challenge \cite{isic2019}, which includes eight dermatological diseases. We use the metadata from this dataset to split this dataset based on gender and age to exam the model fairness in these two dimensions.
\textit{\textbf{Dataset:}} We employ a canonical dataset from the ISIC challenge \cite{isic2019}, encompassing eight dermatological diseases. Utilizing the metadata from this dataset, we segment it based on gender and age to scrutinize the DNN's fairness across these dimensions.


% \textit{\textbf{B. FLNAS settings:}} In evaluating each searched neural architecture from FLNAS, we use $5,000$ out of $25,331$ images. In the $5,000$ images, we make sure the sample sizes of each demographic group are balanced to eliminate the possibility of model performance is conduct from richness of training data or poor of training data. We split the samples into training set with 70\% images, validation set with 20\% images, and test test with 10\% images. We use the model performance on validation set to guild the model training process. During the experiments, we give 10 search attempts for FLNAS. We use a single Nvidia-A10 GPU to evaluate each searched model. 
\textit{\textbf{FLNAS Settings:}} For evaluating each neural architecture derived from FLNAS, we randomly select $5,000$ images from the total of $25,331$ images as the images we use to evaluate the LLM searched DNN architectures. Within these $5,000$ images, we ensure a balanced representation of each demographic group to mitigate the potential bias stemming from the richness or poverty of training data. The dataset is partitioned into a training set with 70\% of the images, a validation set with 20\% of the images, and a test set with 10\% of the images. The DNN performance on the validation set guides the training process. During the experimentation phase, we afford 10 search attempts to FLNAS. A single Nvidia-A10 GPU is utilized to evaluate each searched DNN.


% \textit{\textbf{C. Existing models:}} We select five SOTA works and use them as baselines to compare with the model searched by FLNAS. Four of them are ResNet-18 \cite{he2016deep}, ResNet-34 \cite{he2016deep}, MobileNetV1 \cite{howard2017mobilenets}, and MobileNetV2 \cite{sandler2018mobilenetv2}. They are classical and robust model widely used in image classification tasks. The rest one is FaHaNa \cite{sheng2022larger}, which is a NAS framework to build up fairness model. 
\textit{\textbf{Existing DNNs:}} Five State-Of-The-Art (SOTA) works are selected as baselines for comparison with the DNN generated by FLNAS. Among these, four are ResNet-18 \cite{he2016deep}, ResNet-34 \cite{he2016deep}, MobileNetV1 \cite{howard2017mobilenets}, and MobileNetV2 \cite{sandler2018mobilenetv2}, which are classical and robust DNNs extensively employed in image classification tasks. The remaining DNN, FaHaNa \cite{sheng2022larger}, is a NAS framework designed to construct fairness-enhanced DNNs.


\subsection{Evaluation Metrics}
We evaluate the neural architecture discovered by FLNAS based on hardware efficiency and DNN performance.

% \textit{\textbf{A. Hardware Efficiency:}} There are three metrics that can affect the model deploying. The first metric is number of parameters that can be trained in a model. The more parameters in a model, the better capable the model can learn complicated features. However, we may not always be able to take the advantage of large parameter size when we deploy the model in a resource-limited device. Ideally, the parameter size do not need to be much more than the data complexity requires. Hence, it is valuable and critical to find the proper parameter size, and the smaller parameter size without loss any model performance is the most ideal. Latency is another metric related to hardware limitation. Latency refers to the time the model requires to make one inference. In the device with low computational power, high latency can prevent the model from successfully deploying. In this way, when we search a model, we aim to find the model with lowest latency. Memory space is also pivotal to the model deploying on user-specific devices, where only limited memory space is available to store the model. For the number of parameters, latency, and memory space, we need them to be as small as possible without negatively impact the model performance. 
\textit{\textbf{Hardware Efficiency:}} Three key metrics influence DNN deployment: the number of trainable parameters, latency, and memory space. A higher number of parameters often enables the DNN to learn complex features, although it may not be feasible in resource-constrained environments. Ideally, the parameter size should align with the data complexity. Latency, the time required for one inference, is crucial, especially on devices with limited computational power. Lastly, memory space is essential for deploying DNNs on user-specific devices with limited storage. It is ideal to minimize these metrics without compromising DNN performance.


% \textit{\textbf{B. Accuracy:}} Other than considering the model deployment, evaluate the model performance in complete the given task is important. Accuracy is the most important metric before we consider the model fairness. For example, a model has 30\% of accuracy in all demographic groups given a dataset can lead to a perfect fairness score but the model is still practically incompetent. 
\textit{\textbf{Accuracy:}} Beyond deployment considerations, evaluating DNN performance in completing the given task is crucial. Accuracy is a significant metric before considering DNN fairness. For instance, a DNN with 30\% accuracy across all demographic groups may exhibit perfect fairness, yet remain practically incompetent.


The accuracy is computed as: $\text{Accuracy} = \frac{\sum_{i=1}^{C} \text{TP}_i}{N}$
% \begin{equation}
%     \text{Accuracy} = \frac{\sum_{i=1}^{C} \text{TP}_i}{N}
% \end{equation}
, where \( C \) is the total number of classes, \( \text{TP}_i \) is the number of true positives for class \( i \) (i.e., the number of instances correctly classified as belonging to class \( i \)), \( N \) is the total number of instances.

\textit{\textbf{Fairness:}} As we explained in section 2 part D, unfairness score, EODD, EOPP1, and EOPP2 are used to measure the fairness of given DNN.


% \textit{\textbf{C. Unfairness:}} Fairness is to measure how less bias on all demographic groups a model has in the given dataset. We define a metric called unfairness, which measures how much difference the model perform in each individual group compare to the overall dataset in general. In our metric, the less the value, the less unfair the model, so the fairer it is. To easily demonstrate its mathsmatical concept, we name it unfairness.
% \textit{\textbf{C. Unfairness:}} Fairness gauges the bias across all demographic groups in a dataset. We introduce a metric named unfairness, measuring the performance discrepancy between individual groups and the overall dataset. Lower unfairness values indicate a fairer DNN.


% The unfairness is computed as:
% \begin{equation}
%     \text{Unfairness} = \frac{1}{P} \sum_{j=1}^{P} | \text{Acc}_{j} - \text{Acc}_{\text{overall}} |
% \end{equation}

% where \( P \) is the total number of demographic groups, \( \text{Acc}_{j} \) is the accuracy of the \(j\)-th demographic group, \( \text{Acc}_{\text{overall}} \) is the overall accuracy across all demographic groups.


% % \textit{\textbf{D. Equality of opportunity:}} Equality of opportunity \cite{hardt2016equality} is also a metric related to model fairness issues. It is made to against model discrimination. Different from our unfairness score, which measure the accoracy of each demographic group from high level, equality of opportunity focuses more on the model fairness on positive samples. In detail, there are three metrics under equality of opportunity. The first is equalized odds (EODD). It means, given the same opportunity, the true positive rate (TPR) and false positive rate (FPR) in all demographic groups should be the same. The second is equal opportunity with respect to positive class (EOPP1). Compared to EODD, EOPP1 considers a model fair when the TPR is the same among all demographic groups. The third is equal opportunity with respect to positive class (EOPP2). It considers a model fair when the TNR is the same among all demographic groups.
% \textit{\textbf{D. Equality of Opportunity:}} Equality of Opportunity \cite{hardt2016equality} addresses DNN discrimination. Unlike our unfairness score, which evaluates accuracy across demographic groups, Equality of Opportunity emphasizes fairness concerning positive samples. Under this metric, three sub-metrics exist: Equalized Odds (EODD), Equal Opportunity with respect to the positive class (EOPP1), and with respect to the negative class (EOPP2).
% \begin{itemize}
%     \item \textbf{Equalized Odds (EODD):} This sub-metric asserts that, given the same opportunity, the True Positive Rate (TPR) and False Positive Rate (FPR) should be consistent across all demographic groups. This measure aims to ensure fairness both in favorable and unfavorable outcomes.
%     \item \textbf{Equal Opportunity with respect to the positive class (EOPP1):} Unlike EODD, EOPP1 solely focuses on the fairness in favorable outcomes. It considers a DNN fair when the TPR is consistent among all demographic groups, ensuring that each group has an equal opportunity in receiving positive outcomes.
%     \item \textbf{Equal Opportunity with respect to the negative class (EOPP2):} Conversely, EOPP2 emphasizes fairness in unfavorable outcomes. It deems a DNN fair when the True Negative Rate (TNR) is consistent among all demographic groups, ensuring fairness in avoiding negative outcomes.
% \end{itemize}

% They can be calculated as the following:
% \begin{equation}
%     \text{EODD} = \frac{1}{P} \sum_{p=1}^{P} \max \left( \left| \frac{\text{TP}_{p1}}{\text{P}_{p1}} - \frac{\text{TP}_{p2}}{\text{P}_{p2}} \right|, \left| \frac{\text{FP}_{p1}}{\text{N}_{p1}} - \frac{\text{FP}_{p2}}{\text{N}_{p2}} \right| \right)
% \end{equation}

% \begin{equation}
%     \text{EOPP1} = \frac{1}{P} \sum_{p=1}^{P} \left| \frac{\text{TP}_{p1}}{\text{P}_{p1}} - \frac{\text{TP}_{p2}}{\text{P}_{p2}} \right|
% \end{equation}

% \begin{equation}
%     \text{EOPP2} = \frac{1}{P} \sum_{p=1}^{P} \left| \frac{\text{TN}_{p1}}{\text{N}_{p1}} - \frac{\text{TN}_{p2}}{\text{N}_{p2}} \right|
% \end{equation}

% where \( P \) is the total number of demographic group pairs, \( \text{TP}_{pi} \) is the number of true positives for group \( i \) in pair \( p \), \( \text{FP}_{pi} \) is the number of false positives for group \( i \) in pair \( p \), \( \text{TN}_{pi} \) is the number of true negatives for group \( i \) in pair \( p \), \( \text{P}_{pi} \) is the total number of positive instances for group \( i \) in pair \( p \), and \( \text{N}_{pi} \) is the total number of negative instances for group \( i \) in pair \( p \).

\subsection{Results Analysis}



% In the experiments, we compare FLNAS search models with five SOTA works in two levels of evaluations. To have a better vision of FLNAS capability, we select the four models searched by FLNAS with low unfairness score and high accuracy. We name them as Search-1, Search-2, Search-3, and Search-4. Using the eight metrics we explained in section 4.2, we compare the four searched models with five SOTA models in the same experimental settings. 
In the experiments, we compare FLNAS search DNNs with five state-of-the-art (SOTA) works across two levels of evaluations. To better understand the capabilities of FLNAS, we select top three DNNs searched by FLNAS, characterized by the lowest unfairness scores and highhest accuracy. These DNNs are named Search-1, Search-2, and Search-3. Utilizing the eight metrics described in Section 4.2, we compare these three searched DNNs with five SOTA DNNs under identical experimental settings.


% For hardware efficiency evaluation, the lower the value of each metric for each model, the less hardware resource required to deploy that model. Assuming two models with the same accuracy performance, the model with lower hardware resource requirement is more suitable to deploy to resource-limited device. 
For hardware efficiency evaluation, a lower value of each metric for a given DNN indicates lesser hardware resources required for deploying that DNN. Given two DNNs with identical accuracy performance, the DNN requiring lower hardware resources is more suitable for deployment on resource-limited devices.


% For model evaluation, the higher the accuracy, the more capable the model to make correct classification tasks. Different from accuracy, unfairness, EODD, EOPP1, and EOPP2 are metrics related to fairness. As we explained in section 4.2, the low values of these four metrics reflect the better model fairness. 
In DNN evaluation, higher accuracy signifies a DNN's enhanced capability to correctly perform classification tasks. Unlike accuracy, the metrics unfairness, EODD, EOPP1, and EOPP2 pertain to fairness. As elucidated in Section 4.2, lower values of these four metrics denote better DNN fairness.


% In Table~\ref{tab:evaluation}, we use the notation of \textbf{up arrow} $\uparrow$ and \textbf{down arrow} $\downarrow$ to mark the metric value of each FLNAS searched model if that value is higher or lower to all SOTA works in the same metric. As we can see, the four searched models have more then 10X reduction of the trainable parameters compare to SOTA works, they also have more then 3X latency reductions when they make inference in the given data, and they require more then 10X less memory compare to the SOTA works. Furthermore, the four searched models have up to 11.4\% of accuracy improvement and up to 19X fairness improvement. We highlighted model Search-2, whose performance across all eight metrics is superior than the SOTA works. Especially, for EODD, EOPP1, and EOPP2, they reflect that Search-2 has a fairer performance in classify positive samples than all SOTA works.
In Table~\ref{tab:evaluation}, we employ the notation of \textbf{up arrow} $\uparrow$ and \textbf{down arrow} $\downarrow$ to indicate whether the metric value of each FLNAS searched DNN is higher or lower compared to all SOTA works for the same metric. As observed, the four searched DNNs exhibit more than a 10X reduction in trainable parameters compared to SOTA works, alongside more than 3X latency reductions during inference on the given data, and require more than 10X less memory. Moreover, these DNNs demonstrate up to 11.4\% improvement in accuracy and up to 19X improvement in fairness. We highlight DNN Search-2, which outperforms the SOTA works across all eight metrics. Notably, for EODD, EOPP1, and EOPP2, these metrics indicate that Search-2 exhibits fairer performance in classifying positive samples compared to all SOTA works.


% In execute FLNAS, we only perform 10 search iterations. The total GPU hours costed is 10. Compare to classical NAS frameworks where over 1,000 to 3,000 GPU hours can cost to find a good model, FLNAS is significantly search efficiency. The model it finds also can be hardware efficiency and good performance in accuracy and fairness.
In executing FLNAS, we only perform 10 search attempts, amounting to a total of 3 to 5 GPU hours. This is a stark contrast to classical NAS frameworks, where over 1,000 to 3,000 GPU hours may be expended to find a good DNN. This illustrates the significant search efficiency of FLNAS, which not only finds DNNs more rapidly, but also identifies DNNs that are hardware-efficient and perform well in terms of accuracy and fairness.


% \newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
% \begin{table*}[htbp]
% % \begin{table*}[h!]
% \centering
% \caption{Evaluation of Models}
% \label{tab:evaluation}

% \begin{tabular}{c|c|P{1.7cm}P{1.7cm}P{1.7cm}|P{1.3cm}P{1.3cm}P{1.3cm}P{1.3cm}P{1.3cm}}
% \toprule
% \midrule
% \multicolumn{2}{c|}{\multirow{2}{*}{Model}} & \multicolumn{3}{c|}{Hardware Efficiency Evaluation} & \multicolumn{5}{c}{Model Evaluation} \\
% \cline{3-10}
% \multicolumn{2}{c|}{} & \# of Para. & Latency (ms) & Mem (MB) & accuracy & unfairness & EODD & EOPP1 & EOPP2 \\
% \midrule
% \multirow{5}{*}{\rotatebox{90}{Baseline}} & ResNet-18 \cite{he2016deep}       & 11,169,858 & 0.763 & 2113.91 & 66.67\% & 0.3200 & 0.1077 & 0.0726 & 0.1006 \\
% & ResNet-34 \cite{he2016deep}       & 21,278,018 & 1.450 & 3503.10 & 63.80\% & 0.4354 & 0.1556 & 0.0856 & 0.1335 \\
% % & ResNet-152      & 58,140,226 & 21.800 & 3569.85 & 49.27\% & 1.9157 & 0.0221 & 0.0195 & 0.0148 \\
% & MobileNetV1 \cite{howard2017mobilenets}     & 3,199,106  & 0.594 & 1108.89 & 67.73\% & 0.3498 & 0.1470 & 0.0482 & 0.1287 \\
% & MobileNetV2 \cite{sandler2018mobilenetv2}    & 7,054,850  & 1.563 & 2444.69 & 66.93\% & 0.5778 & 0.1697 & 0.0445 & 0.1620 \\
% & FaHaNa-Fair \cite{sheng2022larger}    & 5,532,866  & 0.644 & 12864.62 & 69.53\% & 0.5591 & 0.1398 & 0.0694 & 0.1267 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{FLNAS}} & Search-1  & $3,309,570 \downarrow$  & $0.273 \downarrow$ & $211.79 \downarrow$  & $75.20\% \uparrow$ & $0.1044 \downarrow$ & 0.1711 & 0.0346 & 0.1711 \\
% & \textbf{Search-2}  & \textbf{293,954 $\downarrow$}    & \textbf{0.155 $\downarrow$} & \textbf{232.88 $\downarrow$}  & \textbf{73.20\% $\uparrow$} & \textbf{0.0306 $\downarrow$} & \textbf{0.0995 $\downarrow$} & \textbf{0.0340 $\downarrow$} & \textbf{0.0995 $\downarrow$} \\
% & Search-3  & $148,098 \downarrow$    & $0.241 \downarrow$ & $158.25 \downarrow$  & $72.00\% \uparrow$ & $0.1136 \downarrow$ & 0.1107 & 0.0204 & 0.1107 \\
% & Search-4  & $420,946 \downarrow$    & $0.286 \downarrow$ & $155.97 \downarrow$  & $73.07\% \uparrow$ & $0.2986 \downarrow$ & 0.1192 & 0.0560 & 0.1183 \\
% \midrule
% % \multicolumn{10}{l}{\small \hspace{1em}1. Arrows indicate performance improvements or reductions compared to all baselines.} \\
% % \multicolumn{10}{l}{\small \hspace{1em}2. Bold font indicates the model with the overall best performance.} \\
% % \multicolumn{10}{l}{\small \hspace{1em}3. Model evaluation is based on the validation set, with the highest accuracy and lowest unfairness selected.} \\
% \bottomrule

% \end{tabular}  % Remember to end the tabular environment

% \end{table*}









% \subsection{Experiment 1: Prompt tuning vs search effectiveness}
% We can compare the prompt format with selective search space, complicated constraints, with simple and high-level descriptions

% For the searched archs, we use them to compare with SOTA

% \subsection{(Maybe?)Experiment 2: Search efficiency }

==> 5_Conclusion.tex <==
\section{Conclusion}
\label{sec_diss}

% In this work, we propose the use of Large Language Models (LLMs) as the replacement of RNN controller in Neural Architecture Search (NAS) to enable efficient neural architecture autonomous design towards fairness and hardware resource efficiency specifically useful in the era of AI democratization. We show the superior performance of FLNAS framework compare to SOTA works. Overall, our work demonstrate the potential of utilize the LLMs in fast design fairness and hardware resource efficient neural architecture. The future investigations can be made in extend the utilization of LLMs in other domain-specific neural architecture design and optimzations.
In this work, we propose the use of LLMs as replacements for the RNN controller in NAS, to facilitate efficient and autonomous design of neural architectures. This approach is particularly beneficial for promoting fairness and hardware resource efficiency, attributes that are critically important in the current era of AI democratization. Our results reveal the superior performance of the FLNAS framework when compared to SOTA works. Overall, our research underscores the potential of employing LLMs for rapidly designing fair and hardware resource-efficient neural architectures. 
% Future investigations could extend the utilization of LLMs to domain-specific neural architecture design and optimizations.

